All-order fluctuating hydrodynamics of the SYK lattice

The SYK model has played an important role in recent developments in many-body quantum chaos. We study a spatially local generalisation of it: the SYK lattice. Starting from the nonlinear action of pseudo-Goldstone bosons that dominate its dynamics at low temperatures, in the long wavelength limit we reorganise this action as the effective field theory for fluctuating hydrodynamics, thereby showing how the hydrodynamic degrees of freedom embed into the microscopic description of the model. We compute the hydrodynamic effective action to high orders in the derivative expansion and determine all the corresponding transport coefficients. Hence this work derives hydrodynamics from the microscopic description of a strongly coupled quantum many-body system.

==> Firstpages.tex <==


% format
\baselineskip=18pt  % a la harvmac
\numberwithin{equation}{section}  % make eq labels (sec.num)
\allowdisplaybreaks  % allow page breaks in displayed eqs


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%        TITLE BEGINS HERE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% ========== title (note version) begins here ==========
%
%\vspace*{-1cm}
%\begin{center}
% {\Large\bf Title of the Document}
%\end{center}
%\vspace*{-.5cm}
%
%% ========== title (note version) ends here ==========

%% ========== title (paper version, a la harvmac) begins here ==========

\thispagestyle{empty}

% Report number if necessary
%\vspace*{-2cm} 
%\begin{flushright}
%{\tt }\\
%\end{flushright}

% title, authors, affiliation
\vspace*{1cm} 
\begin{center}
{\fontsize{20pt}{23pt}\selectfont\textbf{TITLE}\vspace{10mm}}
 
 \renewcommand{\thefootnote}{}
\begin{center}
 \fontsize{14pt}{23pt}\selectfont{}

\end{center}
\vskip .2cm


 \vspace*{.5cm} 
 \fontsize{12pt}{23pt}\selectfont{{$^1$ }}

  
 {\tt {}}

\vspace*{0.8cm}
\end{center}

 \renewcommand{\thefootnote}{\arabic{footnote}}
 
\begin{center} {\bf Abstract } 
\end{center}
Abstract goes here



%%INSERT AN ABSTRACT HERE
\noindent 

%\vspace*{.5cm}

% abstract
%\noindent


\newpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%           TITLE ENDS HERE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\tableofcontents
\printindex

